Survey for Landing Generative AI in Social and E-commerce Recsys -- the Industry Perspectives

Recently, generative AI (GAI), with their emerging capabilities, have presented unique opportunities for augmenting and revolutionizing industrial recommender systems (Recsys). Despite growing research efforts at the intersection of these fields, the integration of GAI into industrial Recsys remains in its infancy, largely due to the intricate nature of modern industrial Recsys infrastructure, operations, and product sophistication. Drawing upon our experiences in successfully integrating GAI into several major social and e-commerce platforms, this survey aims to comprehensively examine the underlying system and AI foundations, solution frameworks, connections to key research advancements, as well as summarize the practical insights and challenges encountered in the endeavor to integrate GAI into industrial Recsys. As pioneering work in this domain, we hope outline the representative developments of relevant fields, shed lights on practical GAI adoptions in the industry, and motivate future research.

==> logistics.tex <==
Mar. 14 -- abstract DDL
Mar. 21 -- tutorial proposal and survey paper DDL

==> paper-agent-DZ.tex <==
\subsection{Research Progress}
GAI enables interactive recommendations by curating human-like responses for various purposes such as direct recommendation, preference refinement, recommended follow-up questions, and recommendation justification \cite{jannach2021survey, huang2024foundation}. To enable such an interactive recommendation system with GAI, the use of an AI agent is required \cite{deng2024large, wang2023recmind}, where the baseline RAG can be considered a simple AI agent with retrieval and generation modules.

LLM-powered agents can utilize an LLM to reason through a problem to create a plan for solving it (planning) and leverage LLMs to produce text-based outputs and actions that can be used for making API calls to utilize a set of tools.
In the planning step, we could generate a pre-defined reasoning graph for the LLM to explore and follow \cite{yang2022seqzero} or use the LLM reasoning capabilities to generate the reasoning path on the fly using frameworks like CoT \cite{wei2022chain} or ToT \cite{yao2024tree}.
In each step, the agent uses LLM to generate textual output for the agent to decide whether or not, and how, to call a tool.

\subsection{Solution Frameworks and Practical Considerations}
There are two types of AI agents, where the main difference lies in how planning is executed: whether it is predefined or generated in real time.

\subsubsection{With pre-defined reasoning graph}

As shown in Figure \ref{fig:rag}, we outline one example of using a pre-defined reasoning graph and allowing LLM-agents to make decisions on how to navigate the graph. For example, when we have an interactive recommendation interface with users, important questions arise: whether we want to rewrite the user prompt, retrieve user history, or recommend or just chat. In many cases, the user prompt itself is sufficient for generation. Suppose the customer simply says "hi" in the interactive recommendation interface; we could use the GAI to generate the response, instead of invoking query rewrite, retrieval, and reranking modules. We have deliberately designed the system this way to reduce latency. Regarding the function calling decision, since the reasoning graph is pre-defined and the task is predefined, we don't need to use an LLM to generate the output for a function call; we could use some simple rules to decide, or we could use a lightweight model for decision-making.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{images/RAG-agent.png}
    \caption{Proposed GAI agent with pre-defined reasoning graph}
    \label{fig:rag}
\end{figure}


\subsubsection{Use GAI for planning}
In \cite{wang2023recmind}, the authors describe one example of how to use an LLM to generate the reasoning path on the fly using a self-inspiring (SI) planning technique and compare the performance with CoT \cite{wei2022chain} and ToT \cite{yao2024tree}. The interactive agent also allows the use of several tools, including (1) database tools that enable text2sql and SQL execution, which allows us to tackle computationally intensive tasks, answering questions like "What is the average rating of a product?" and "What's the top 5 cheapest products", (2) a web search tool when the information is not available in existing databases, (3) and a text summarization Tool. The agent also has a memory module, which is a crucial pathway to enhance planning capabilities \cite{huang2024understanding}.

From a practical perspective, open-source fine-tuned models still lack the capacity to enable Type 2 GAI agents, and most work in this area is built on top of closed-source ChatGPT or Claude APIs \cite{wang2023recmind}. On the other hand, Type 1 GAI agents could be powered by some fine-tuned open-source LLM models. On the other hand, creating a predefined reasoning graph requires domain expertise and might not be optimal for all cases. This means the response will be subpar for some user inputs.



==> paper-agent.tex <==
\subsection{Research Progress}
The recommendation system (RecSys) has been significantly improved through the integration of Deep Neural Networks (DNNs), exemplified by Deep & Cross Network (DCN)\cite{wang2017deep}, and pre-trained Large Language Models (LLMs), such as BERT\cite{gregory2008mir}, to more effectively learn the representations of users, items, and sequential behaviors. However, current methodologies are hampered by their inability to adequately capture textual knowledge pertaining to users and items, due to constraints in model scalability and data volume\cite{fan2023recommender}. Furthermore, the majority of existing RecSys approaches are tailored for specific tasks, demonstrating a lack of generalizability to novel recommendation scenarios. Additionally, these methods often fail to leverage external tools for accessing real-time information and external knowledge bases, which limits their effectiveness. The absence of reasoning capabilities in current Recsys approaches results in suboptimal recommendation outcomes\cite{liu2023chatgpt}. To address these shortcomings, we advocates for the augmentation of RecSys with LLMs, harnessing the robust reasoning capabilities and tool utilization proficiency of LLMs, in conjunction with the information retrieval framework discussed in preceding sections. We describe an LLM-based RecSys agent, detailing its architecture and essential components.

\subsection{Solution Framework}
Consistent with the framework outlined by\cite{wang2023survey}, we conceptualize a LLM-based Recsys Agent as comprising several key modules: a profiling module, a memory module, a planning module, a tools module, and an action module. This structure is designed to endow the agent with a comprehensive set of capabilities, facilitating nuanced and effective recommendation processes. Each module plays a critical role: the profiling module define the characteristics of the agent; the memory module stores and retrieves information and past interactions; the planning module strategizes the recommendation steps; the tools module leverages external resources; and the action module executes the recommendations. Together, these components work in concert to simulate a sophisticated, human-like decision-making process within the RecSys Agent~\ref{fig:gai-agent}.


\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{images/gai-agent.png}
    \caption{A framework for the architecture design of LLM-based GAI agent.}
    \label{fig:gai-agent}
\end{figure}

The Recsys Agent's profiling module typically encompasses demographic details, including name, gender, and age, alongside psychological information that mirrors the personalities of the agents, and social data elucidating the interrelationships among agents. The selection of information for profiling the agent is predominantly dictated by the application scenarios. The profiling module may be deemed optional in the construction of an agent for a recommendation system, while the strategic design of system prompts for tasks entailing role play, such as "Assuming you are an expert recommending products to users, ...," could potentially enhance the task's performance and precision in practical applications. 

The Recsys Agent's memory module is designed to simulate human memory, comprising both short-term and long-term components. Short-term memory, typically facilitated by in-context learning, forms an integral part of the system's prompts. This allows for the incorporation of examples and reasoning for guidance, the inclusion of edge cases, or the retrieval of users' historical conversations via in-memory techniques, such as memory buffers or online key-value databases. Despite its efficacy, short-term memory is constrained by the context window limitations of LLMs, making it challenging to incorporate all pertinent memories or data into a single prompt. This limitation can adversely affect agent performance, underscoring the necessity for long-term memory. Long-term memory serves to store relevant documents and items, past interactions, historical data, etc, enabling retrieval in response to user's queries. Techniques such as RAG system and external vector databases are employed as mechanisms of long-term memory, retrieving relevant information through embedding similarities. This bifurcated approach to memory—encompassing both short-term and long-term elements—ensures a more dynamic and comprehensive interaction capability for RecSys Agents, aligning closely with the complexities of human memory and cognition.

The Recsys Agent's planning module is designed to equip the agents with capabilities akin to human cognitive processes. The planning model facilitates the agent's ability to deconstruct complex tasks, such as those encountered in recommendation scenarios, into manageable segments. This decomposition is achieved through methodologies such as the Chain of Thought\cite{wang2022self}, Tree of Thought\cite{yao2024tree}, Reflection\cite{shinn2024reflexion}, self-critics\cite{gou2023critic}, subgoal-decomposition\cite{liang1990problem}. These approaches, enable agents to efficiently navigate and address complex situations within the context of recommendations. Through the implementation of these strategies, RecSys Agents are better prepared to handle the intricacies and dynamism inherent in recommendation tasks, thereby enhancing their performance and utility.

The Recsys Agent's tools module designed to facilitate effective utilization of tools and interaction with external APIs. This module could enhances the capabilities of RecSys agents, particularly in domains that require extensive expert knowledge, or in addressing the hallucination issues commonly associated with LLMs. For example, an agent might leverage the tools module to invoke a knowledge graph API or a web search function call. This enables the agent to gain a deeper understanding of the entities and contents present in a user's query, thereby improving the quality and accuracy of its responses and recommendations. Through this mechanism, the tools module serves as a crucial component in bridging the gap between the innate capabilities of LLMs and the dynamic, information-rich environment, enhancing the overall effectiveness of the RecSys agent.

The Recsys Agent's action module, guided by inputs from the profiling, memory, planning, and tools modules, interacts directly with the environment by transforming the agent’s decisions into tangible outcomes. This integration is crucial for the operational efficacy of the RecSys Agent, ensuring a smooth transition from decision-making to the execution of actions. Furthermore, in contrast to traditional RecSys approaches that merely deliver recommendations in response to user queries, the action module enables an interactive RecSys Agent to engage with the user. This engagement allows the agent to solicit additional personal preferences and background information, thereby refining the decision-making process.

==> paper-curation.tex <==


\subsection{Research Progress}
GAI enables interactive recommendations, wherein it curates human-like responses for multiple purposes such as direct recommendation, preference refinement, recommended follow-up questions, and recommendation justification \cite{jannach2021survey, huang2024foundation}. The baseline system that enables such an interactive recommendation system is the use of RAG (Retrieval-Augmented Generation) \cite{lewis2020retrieval}, where the baseline RAG can be regarded as a simple AI agent with retrieval and generation modules. 

RAG \cite{lewis2020retrieval} aims to address outdated knowledge, the generation of incorrect information (hallucinations), and limited domain expertise by combining the LLM’s internal knowledge with dynamic external knowledge bases.
RAG-based Recommender Systems combine the strengths of retrieval-based and generation-based models to enhance the ability of RSs to provide relevant suggestions \cite{di2023retrieval}.
RAG is a rapidly developing area that includes self-RAG, auto-RAG, and Corrective RAG, focusing on adding more modules to the general retrieval-generation workflow. This includes adding components like retrieval result verification and reranking \cite{yan2024corrective, zhuang2023open, li2023llatrieval}, adaptive retrieval \cite{jiang2023active}, and query rewrite \cite{ma2023query}.

\subsection{Solution Framework}


As shown in Figure \ref{fig:rag}, we outline the RAG modules for GAI curation. When we have an interactive recommendation interface with users, important questions arise: whether we want to rewrite the user prompt, whether we want to retrieve user history, and whether we want to recommend or just chat. For many cases, the user prompt itself is sufficient for generation. Suppose the customer simply says "hi" in the interactive recommendation interface; we could use the GAI to generate the response, instead of invoking query rewrite, retrieval, and reranking modules. We have deliberately designed the system this way to reduce latency. Regarding the function calling decision, we could use some simple rules to decide, or we could use a lightweight model for decision-making. It is also recommended to use LLMs only when necessary to reduce latency costs and to adopt pretrained or finetuned smaller models for other functional modules. For example, instead of using LLMs to rerank first-stage retrieval results, we could use reranker models like FlashRank \cite{Damodaran_FlashRank_Lightest_and_2023} and Cohere Reranker\cite{cohere_rerank_multilingual_v2_0}.


The proposed framework also aims to capture both short-term and long-term user preferences. For short-term preferences, the system can save or summarize conversations as a temporary memory to capture immediate interests. For long-term preferences, it can employ a dedicated retriever to retrieve relevant portion of the user's interaction history \cite{lin2023rella}, identifying enduring interests. This dual approach leverages RAG's capabilities to offer timely and personalized recommendations, balancing immediate context with historical user behavior for enhanced personalization.



\begin{figure*}[htb]
    \centering
    \includegraphics[width=1\textwidth]{images/RAG.png}
    \caption{Proposed RAG system for GAI curation}
    \label{fig:rag}
\end{figure*}

